The Coherent Magnetic Field of the Milky Way

We present a suite of models of the coherent magnetic field of the Galaxy (GMF) based on new divergence-free parametric functions describing the global structure of the field. The model parameters are fit to the latest full-sky Faraday rotation measures of extragalactic sources (RMs) and polarized synchrotron intensity (PI) maps from WMAP and Planck. We employ multiple models for the density of thermal and cosmic-ray electrons in the Galaxy, needed to predict the skymaps of RMs and PI for a given GMF model. The robustness of the inferred properties of the GMF is gauged by studying many combinations of parametric field models and electron density models. We determine the pitch angle of the local magnetic field (11+/-1 deg.), explore the evidence for a grand-design spiral coherent magnetic field (inconclusive), determine the strength of the toroidal and poloidal magnetic halo fields below and above the disk (magnitudes the same for both hemispheres within 10%), set constraints on the half-height of the cosmic-ray diffusion volume (>2.9 kpc), investigate the compatibility of RM- and PI-derived magnetic field strengths (compatible under certain assumptions) and check if the toroidal halo field could be created by the shear of the poloidal halo field due to the differential rotation of the Galaxy (possibly). A set of eight models is identified to help quantify the present uncertainties in the coherent GMF -- spanning different functional forms, data products and auxiliary input, and maximizing the differences in their predictions. We present the corresponding skymaps of rates for axion-photon conversion in the Galaxy, and deflections of ultra-high energy cosmic rays.

==> dataAndModels.tex <==
\begin{figure*}[ht]
  \modelPlot{pics/Models/JF12CoherentConfig}{JF12Disk}{JF12Toroidal}{JF12Xfield}
  \caption{Predictions for \RM, \Q and \U of the default JF12 model.
    The predictions from the individual model components are shown
    in the top rows, followed by full model prediction.}
\end{figure*}
\begin{figure*}[ht]
  \modelPlot{pics/Models/uf23_base}{FourierDisk}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_base}
    \fitPlotCaption{\modelBase}
\end{figure*}
\begin{figure*}[ht]
    \modelPlotTwist{pics/Models/uf23_twist}{FourierDisk}{TwistedXfield}
    \fitPlot{pics/Fits/uf23_twist}
    \fitPlotCaption{\modelTwist}
\end{figure*}
\begin{figure*}[ht]
    \modelPlot{pics/Models/uf23_xr}{FourierDisk}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_xr}
    \fitPlotCaption{\modelXr}
\end{figure*}
\begin{figure*}[ht]
    \modelPlot{pics/Models/uf23_spur}{SpiralSpur}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_spur}
    \fitPlotCaption{\modelSpur}
\end{figure*}
\begin{figure*}[ht]
    \modelPlot{pics/Models/uf23_ne}{FourierDisk}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_ne}
    \fitPlotCaption{\modelNe}
\end{figure*}
\begin{figure*}[ht]
    \modelPlot{pics/Models/uf23_kappa}{FourierDisk}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_kappa}
    \fitPlotCaption{\modelKappa}
\end{figure*}
\begin{figure*}[ht]
    \modelPlot{pics/Models/uf23_cre}{FourierDisk}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_cre}
    \fitPlotCaption{\modelCre}
\end{figure*}
\begin{figure*}[ht]
    \modelPlot{pics/Models/uf23_syn}{FourierDisk}{JF12Toroidal}{CoastingXfield}
    \fitPlot{pics/Fits/uf23_syn}
    \fitPlotCaption{\modelSyn}
\end{figure*}

